Navigo: Interest Forwarding by Geolocations in Vehicular Named Data Networking

This paper proposes Navigo, a location based packet forwarding mechanism for vehicular Named Data Networking (NDN). Navigo takes a radically new approach to address the challenges of frequent connectivity disruptions and sudden network changes in a vehicle network. Instead of forwarding packets to a specific moving car, Navigo aims to fetch specific pieces of data from multiple potential carriers of the data. The design provides (1) a mechanism to bind NDN data names to the producers' geographic area(s); (2) an algorithm to guide Interests towards data producers using a specialized shortest path over the road topology; and (3) an adaptive discovery and selection mechanism that can identify the best data source across multiple geographic areas, as well as quickly react to changes in the V2X network.

==> LocationIndependentDesign.tex <==
\section{Location-independent data: Where is the content?}
\label{sec:locIndependent}
Although in vehicular scenario a large class of application is intrinsically location dependent, not all the information a car (or the driver) is interested about have a relation with a specific location, i.e news, music, .... These classes of data don't come with a geographical meaning, nevertheless \name proposes a self-learning scheme to discover and then exploit the geographical area where these ``location-independent'' Interest are more likely to be satisfied, such as areas where a RSU can be found or areas with other cars carrying the desired data in their caches.
Specifically, \nameNoSpace: (1) creates a binding between the content location and the content name; (2) provides the producer's applications with a mechanism to register routable prefixes on the network; (3) exploits the binding between names and geographical location to guide the interest towards the content along the best path.
The main concept \name exploits is the following: after getting few chunks of an information from a node (either access point that provide Internet connectivity or another car), and therefore from a certain location, it's likely that in the short term interest for different chunks of the same information will be satisfied in the same area, likely from the same node.
%% LZ: "routable prefix"?? You mean "reachable"?


\subsection{How to Find Data Source Locations}
With location-independent application a car has no clue where the requested data may resides. \name proposes an initial \emph{exploration phase}, during which the node broadcasts Interests on the V2V network using a controlled flooding mechanism as in \cite{2014NOM-VNDN} to locate any available data source. As soon as the consumer recovers the first Content, it starts sending next Interests focusing only on the most promising direction, the location of the data provider, instead of keeping flooding the network.
%Binding a content with a location requires the node to know where this data can be found. If a car has no clue where the requested data may resides, one simple approach adopted by \cite{2014NOM-VNDN} is to broadcast Interests on the V2V network using a controlled flooding mechanism and then waiting for the content, which will follow the breadcrumbs left by the Interest in the PIT of the forwarding nodes. \name extends this approach by enabling Contents to carry information about the locations of the node that is providing the data, so that future Interests can focus on most promising direction instead of flooding or randomly spread. 
%\begin{itemize}[noitemsep,topsep=2pt,parsep=0pt,partopsep=2pt]
%	\item A producer (if it's a vehicle);
%	\item A car that is providing data using its cache;
%	\item An access point which is forwarding the content from the Internet to the V2V network;
%	\item A car that is forwarding the content from the Internet (using for example a 3G or 4G device) to the V2V network. 
%\end{itemize}
 
\subsubsection{Binding Content Location to Names}
Whenever a Content ``enters'' the V2V network, the location of the node that is providing the data (either the producer, a mule or an Internet access point) is attached to a 2.5 layer header defined by LAL to encapsulate NDN packets. 
 %More in details, the LAL encapsulates NDN packets in a 2.5 layer which carries the pair \textbf{$<$prefix of the content : location of the node$>$}, thus allowing the consumer and all the intermediate nodes to learn the location of the node who is providing the Content. 
When a car receives a data packet with a location attached, it creates a virtual geo-faces associated with the area where the Content is coming from (if such face is not already available) and then it registers the prefix of the Content in the FIB, binding the GeoFace with the information retrieved. Interests for the next chunk of that information will then be sent through that specific GeoFace and thus toward the same area ...TODO \todo{answer the question: why do we use areas instead of specifying the coordinates of the destination}
While in our experiments \name uses this approach only for location independent application, by design \name can enable a node which is running location dependent application to use the hints provided by the consumer and by the data source in conjunction, bounding the same prefixes to multiple faces.%, as shown in \ref{sec:ForwardingAlg}.

\subsubsection{Routable prefixes}
While the whole name of the data packet identifies the specific part of the information the packet is carrying, usually by a sequence number or a timestamp as last component of the name, only part of the name is needed to identify the whole information the consumer is looking for.
For instance, receiving the piece of a song ``/spotify/songA/chunk10'', the prefix /spotify/songA identifies the whole information, the song, while the complete prefix with the chunk number identifies a specific piece of that song (chunk 10). In this case, only the prefix /spotify/songA (so-called \emph{routable prefix}) has to be bound to the GeoFace which received the data, so that every interest with the prefix ``spotify/songA/chunkY'' will be sent to that area, no matter which chunk Y the Interest is asking for (forwarding rules in FIB match names by longest prefix match: both interests with names \emph{/spotify/songA/1} and \emph{/spotify/songA/2} match the rule \emph{/spotify/songA}). \note{should we put a reference to the FIB longest prefix match?}


%As shown in this example, the node won't register the whole name of the content, but just a part of it, the part that specifies the name of the application and the title of the song, without the chunk number. Indeed the chunk number specifies only a small part of the information, while it's ``spotify/songA'' that identifies the entire information the user in interested on. By registering the whole name of the content with the chunk number in it in the FIB, the forwarding rule will match (longest prefix matching) only Interest for that that specific segment, while Interest for different chunks of the same song won't match the rule and therefore won't be sent to the right destination area. Only by bounding the prefix that identifies the whole information (spotify/songA''), the so called \textbf{routable prefix}, to the GeoFace associated to \emph{X}, all the interest for that song will be sent towards the correct destination area.


Consumers and producers know the semantic of the name, therefore they can tell the local NDN daemon which part of the name identifies the whole information, which is the routable prefix. In contrast, the forwarders are unaware of the meaning of the name and thus are not able to identify the routable prefix by themselves\footnote{Assuming that only the last component of the name identifies the specific chunk of information might not be always true.}. To address this problem, the data source attaches to the L2.5 metadata that encapsulate the Content not only its location, but also the ``routable'' prefix of the data (/spotify/songA), which can be used by the forwarders to learn from the network and fill up their FIB (the LAL takes care of extracting the information from the packet and registering the routable prefix in the FIB). 

%While in the nodes where producer or consumer are running, the application can tell the NDN daemon which part of the name identifies the whole information, which is the routable prefix, the nodes that take care of forwarding Interests and Contents are unaware of the meaning of the name and therefore are not able to identify the routable prefix by themselves. 

%Data producer\footnote{this can be also a cache} attaches to data packets the pair of prefix:region, thus allowing the consumer and all the intermediate nodes to learn the data location; 
In summary, when a Content comes back it carries the routable prefix and the source coordinates via the L2.5 metadata. For instance, when sending a chunk of song with the name \texttt{/spotify/songA/chunkN} from the location \emph{4QFJ 1234 5678}, the provider of the data attaches the pair \emph{$<$/spotify/songA , 4QFJ 1234 5678$>$} to the L2.5 metadata. Each cars, receiving the Content, registers the prefix in the FIB as $<$spotify/songA:GeoFaceID$>$ while the mapping between GeoFaceIDs and the region where the content location 4QFJ 1234 5678 is located is kept within the NDN-V2X adaptation layer. 

By allowing the forwarder nodes to fill up the FIB with the information about the routable prefixes, at each hop the car is able to autonomously decide to send the interest based on the consumer will or based on the information present on its own FIB. While in our experiments forwarders always follow consumer's will, by design every \name node is able to forward the Interest toward a different area if it thinks that its information are more trustworthy than the indication provided by the consumer. The benefits and the possible challenges that this approach could bring are left for future works.


\subsection{Forwarding algorithm}
\label{sec:ForwardingAlg}
Content can be retrieved by different locations and therefore by different GeoFaces.
Having multiple choices to retrieve an information brings multiple benefits, such as reliability in case of route failure and traffic load balancing, but it also introduce the new challenge of choosing among all the available faces. Furthermore, in contrast with the wired scenario, the highly dynamic nature of vehicular networks limits the validity in time of forwarding rules and requires the FIB to be updated at higher rate to avoid sending interest to the wrong or less efficient area. 
To address the staleness problem while exploiting the multipath capabilities of such scenario, \name adopts the following strategy:
\begin{itemize}
\item \name maintains a list of \emph{available faces} for each routable names it encounters
\item Whenever it receives a Content with a routable name \emph{N} from a GeoFace X, it adds the face to the list of \emph{available faces} for \emph{N}.
\item When a node has to send an Interest, it uses one of the geoFaces in the \emph{available faces} list in a round robin way.
\item Whenever an Interest is sent using a geoFace F\_X, if F\_X doesn't receives the requested content before a deadline T (300ms in our experiments), F\_X is removed from the \emph{available faces} list.
\item If the list is empty (there are no information available about the location of the content), the Interest is sent using a controlled flooding technique (see \ref{sec:LAL}) without specifying any destination area - the node is in a so-called \emph{exploration phase}.
\item If the list has only 1 element, with a probability \emph{p} (0.95 in our experiments) the node uses the geoFace in the list, while with a probability 1-{p} the node acts as in the \emph{exploration phase}, flooding the interest in all the directions. \name adopts this additional exploration phase to (1)avoid focusing on only one destination area for a long time while some other opportunities might come with mobility to balance the traffic, (2) limit the number of times the \emph{available faces} list is empty (in such cases, before being able to send interest to a specific area, the node has to wait at least an entire round trip time; during such time all the interest the node sends will be spread in all the directions).
\end{itemize}


%\begin{algorithm}[]
%\tcc{Forwarding Interest I}
%\KwData{Interest \emph{I}, Available geoFaces for \emph{I} \emph{availableGeoFaces}}
%{
%	\uIf{$isEmpty(availableGeoFaces)$}{
%		\tcc{No available information; \emph{Exploration Phase} }
%		Send \emph{I} using \emph{V2VFace} 
%	}
%	\uElseIf{$ Size(availableGeoFaces) = 1$}{
%		$ExplorationProbability \longleftarrow $UniformRandom(0:1)\;
%		\eIf(\tcc*[f]{Exploration Phase}){$ExplorationProbability < \epsilon$ }{
%			Send \emph{I} using \emph{V2VFace} 
%		}
%		{
%			$geoFace \longleftarrow $GetNextRoundRobinFace(availableGeoFaces)\;
%			Send \emph{I} using \emph{geoFace}\;
%			SetTimeout for \emph{geoFace}\;
%		}
%	}
%	\Else{
%		$geoFace \longleftarrow $GetNextRoundRobinFace(availableGeoFaces)\;
%		Send \emph{I} using \emph{geoFace}\;
%		SetTimeout for \emph{geoFace}\;
%	}
%}
%***********************************************
%\tcc{Receiving Content \emph{C}}
%\KwData{Content \emph{C}, geoFaces {F}}
%{
%	$R \longleftarrow RoutableNameOf(C)$\;
%	$geoFaceByName \longleftarrow GetFacesFor(R)$\;
%	 \eIf{$F \in geoFaceByName$}{
%		$RemoveTimeout(R,F)$\;
%	}
%	{
%		Add \emph{F} to FacesFor \emph{R}\;
%	}
%}
%***********************************************
%\tcc{Interest Expiration}
%\KwData{Routable name \emph{R}, geoFaces {F}}
%{
%	Remove \emph{F} from FacesFor \emph{R}\;
%}
%\label{alg:ForwardingByGeoFaces}
%\caption{Forwarding process using GeoFaces}
%\end{algorithm}
%\todo{algorithm. show that exploration phase use the v2vFace to flood the interest in all the directions. It might be the first time the v2v face is mentioned in the paper. check this out}

\section{FIB Management}
%{\todo{ADD SOME CONSIDERATION ON THE FIB/FACEs Scalability i.e. we just need to keep information about regions that are few hops away.}
%scalability concern
%rules lifetime
\label{sec:FibManagment}
Each FIB entry stores the routable prefix and a list of faces that can be used to retrieve such Content. Associating geographic areas with faces, the region's dimension could affects the size of the FIB: indeed decreasing the size of these areas increases the probability to have multiple geoFaces bounded to the same routable name, especially when the data source is a moving car: whenever a car that is providing data migrates from a region to another, the consumer receives data packets from a different area and therefore from a different geoFace, increasing thus the number of faces associated to the same routable prefix. On the other end, if the region is too large, the FIB will be smaller but the portion of area where cars will forward the Interest in all the available directions increases, leading to a larger overhead. 
Preliminary result showed 200x200 meters as good tradeoff for the size of the region associated with a geoFace. Future analysis will investigate more accurately the effects of the area's size and the possibility of having regions with different size.
Anyway it must be noticed that removing a GeoFace from the list of available faces for a routable prefix as soon as an Interest fails doesn't allow such list to grow uncontrollably.
%To prevent the FIB to keep growing, rules with low revenue levels and rules that have not been updated recently might be removed from the FIB. Furthermore, rules about traffic generated by a local application might have a longer lifetime in the FIB compared to rules concerning information that the node has simply forwarded.


%How long to keep the FIB entries from self-learning?

%by default, just store it in the forwarders for a short period of time. 



%distinguish producers of vehicles and producers residing on Internet infrastructure. Information attached to Data packets by RSUs can have long lifetime.

==> VANET-Characteristics.tex <==
\section{Vehicular Networks and Applications}
%% LZ: exactly how many points does this section intend to make?

Vehicular networks are dynamic systems where nodes move frequently through the urban maze of roads and artifacts or they quickly pass by a stretch of high speed motorways. Node mobility and urban obstacles cause frequent link disruptions and sudden changes in network topology.
Previous work~\cite{rowstron2009characteristics} analyzed the vehicle-mobility of the city of Portland, Oregon during morning rush hour to understand VANET's dynamics. 
In the Portland scenario, the link duration is less than 10 seconds in 97\% of the cases.
% and some nodes are always disconnected. In short, vehicular networks are dynamically partitioning systems. 
Traditional network design principles do not hold in the VANET case, network protocols and applications need to be able to cope with disruptions and frequent topology changes. 

IPÕs node-to-node communication encounters several difficulties in the vehicular scenario due to frequents and sudden topology changes and disruptions in the communication. NDN by focusing on contents instead of nodes, can bring substantial benefits in such scenarios~\cite{2014NOM-VNDN}. 
%% LZ: repetition again
In NDN applications name the data. Application names are used by the network in lieu of "addresses" directly. The Named Data network architecture was first introduced in \cite{VanSmThPlBriBra09-Networking} and identified three main types of network elements: producers, consumers, and routers. On the wire NDN entails two different types of packets \emph{Interest} and \emph{Data}. NDN nodes use interest packets to request a specific \emph{named data} from the network while \emph{data packets} contain the actual data associated with a specific \emph{name}. To perform routing and forwarding each NDN node maintains three major data structures: Content Store (CS), Pending Interest Table (PIT), and Forwarding Information Base (FIB). The CS caches \emph{data packets} received and that are potentially useful to satisfy future \emph{interest packets}. The PIT stores \emph{interest packets} that have been forwarded to the network but are not yet satisfied by any incoming \emph{data}. The FIB is the NDN equivalent of IP routing tables; i.e. if an \emph{Interest} finds no match in either the CS or the PIT, it will be forwarded toward the data producer(s) according to the FIB (which is maintained by a name-based routing protocol). On the data path, when a \emph{data packet} arrives, the router finds the entry in the PIT that matches the \emph{data name} and forwards the data to all downstream interfaces listed in the PIT entry. It then removes that PIT entry, and caches the Data in the CS. If a \emph{data packet} does not have a matching PIT entry, it is unsolicited and is dropped. It is important to note that neither Interest nor Data packets carry IP addresses; Interest packets are routed toward data producers based on the names carried in them, and Data packets return based on the state information set up by the Interests at each hop.
%% LZ: a basic NDN intro is needed, but should ONLY mention the points that are relevant to this paper.

\cite{2014NOM-VNDN} shown the feasibility of a NDN deployment in the vehicular scenarios, but as stated in the paper, it was just a proof of concept. The approach of blindly flooding (even if it's done by using a controlled flooding mechanism) the V2V network all the time to retrieve the data is not sustainable in a dense scenario, due to the high overhead of the communication. Therefore, a mechanism to discover the content position and steer the packet forwarding only in that direction to limit the overhead is needed. 
%%
While having a omniscient centralized infrastructures on the Internet that provides either the content itself or its position might seem a good solution, relying on such infrastructure might not be always feasible: (1) the cost for the user to be always connected to such infrastructure (i.e. with 3G/4G connection) is not negligible; (2) the cost to maintain the information provided by a central server up to date might be high since cars have to periodically communicate their position; (3) a centralized approach is usually affected by scalability issues. \\
\name addresses such problems and proposes a mechanism to discover the location of the content and efficiently retrieve it over V2V communication without relying on a centralized infrastructure.
%% LZ: do we really need this "centralized infrastructure" discussion here??
%%
%Furthermore, knowing the location of a content addresses only part of the problem. The content must be retrieved - cars have to efficiently propagate the request for the data exploiting the cost-free car to car communication and then get back the content.


%\todo{Introduction of the main problems that we aim to solve: without an infrastructure, we don't know where the content can be found. Flooding all the time is not a sustainable solution, rely on the infrastructure to locate the content is expensive (cost per pkt + cost for server ...). Cars can be an important component in the communication, not only as end user of the data, but also as a mean to produce, deliver and carry the content, but we need a protocol that enable these underutilized capabilities  }
Applications on a running car include traditional Internet applications as well as specific vehicular applications including safety alerts, parking, traffic jam notifications, applications. The first class of applications requires either a direct or indirect Internet access (through access points, other cars, or caches); the later features a natural binding between the application semantics and geographic areas. In both cases the geographic location either of the data itself or of the Internet access point can be exploited for protocol and application design.
\name proposes to exploit this natural binding among data and geographical location for the second class of application by:
%\name is a geographic-based forwarding scheme for V2X scenarios that proposes to exploit this binding between data and geographical location for the latter application by:
\begin{itemize}
	\item enabling such location-dependent application to inform the node of the location of interest;
	\item Introducing a mechanism to efficiently steer the interest flooding toward a specific geographical area of interest along a well defined path computed on the road-topology using a modified Dijkstra algorithm.
\end{itemize}
Furthermore, \name proposes to find a binding among data and geographic areas even for traditional location-independent applications and then exploit such binding to steer the interest. \name proposes to explore the area around a car to locate either a Internet point of access (i.e. RSU) or another car which is carrying the requested data and then temporarily bind the data with such location. Due to the highly dynamism of vehicular network, this binding can be broken by cars movement; therefore \name defines a mechanism to efficiently update the binding and react to changes in the topology. 
%%
%% LZ: the above is a mix of things that don't seem to belong here: (1) 

%To adapt NDN to the VANET characteristics and exploit them \name extends the Link Adaptation Layer (LAL) protocol described in \cite{2014NOM-VNDN} which addresses the problematic of a highly dynamic environment such as VANET, while taking full advantage from the broadcast nature of the wireless channel. 

%\name  is a geographic-based forwarding scheme for V2X scenarios which includes a  Link Adaptation Layer (LAL) protocol built on the protocol described in \cite{2014NOM-VNDN}. \name introduces mechanisms to bind data to its location  and to geographically steer  interest forwarding to a well defined path computed on the road-topology using a modified Dijkstra algorithm.

%\subsection{Identifying locations}
%We divide the world into regions according to the Military Grid Reference System (MGRS)~\cite{mgrs}, where each region is identified by a label. The MGRS is derived from the Universal Transverse Mercator (UTM) grid system and the Universal Polar Stereographic (UPS) grid system, but uses a different labeling convention. The MGRS is used for the entire Earth. An example of an MGRS coordinate, or grid reference, would be \emph{4QFJ12345678}, which consists of three parts: \emph{4Q} (grid zone designator, GZD); \emph{FJ} (the 100,000-meter square identifier); \emph{12345678} (numerical location, where easting is \emph{1234} and northing is \emph{5678}). In this case it specifies a location with 10m resolution, while \emph{4QFJ1234567890} would identify the same location with a 1m resolution.  The number of digits in the numerical location must be even: 0, 2, 4, 6, 8 or 10, depending on the desired precision. Euclidean geometry holds within a region, therefore computing distances, headings or coordinates is trivial (a grid example in figure \ref{fig:mapgrid}).
%\begin{figure}
%%\vspace{-0.18in}
%\begin{minipage}[t!h]{\columnwidth}
%\centering
%\includegraphics[width=0.7\columnwidth]{MapwithGrid.png}
%%\vspace{-0.4cm}
%\caption{Map with grid}
%\label{fig:mapgrid}
%\end{minipage}
%\vspace{-0.2in}
%\end{figure}
%
%\subsection{Mapping Names to Geographical Areas}
%\name introduces the concept of Geographical-Faces (GeoFaces) to bind the data to the geographical grid. Each GeoFace represents an Area according to reference geographical grid.  GeoFaces are labeled and stored in \name Link Adaptation Layer (LAL).  Specifically,  \name link adaptation layer keeps a \emph{GeoMapping} table to map regions~$\rightarrow$~GeoFace(s) that is used to support interest forwarding decisions and reduce probability of spreading the interest in areas less likely to contain the requested data. 
% 
%\name LAL specifies a protocol used to register prefixes and bind them to GeoFaces without requiring (intermediate) nodes to understand the name semantics. In particular, when a content is found, \name stores the name-prefix and its location information in the LAL header and carries it back as metadata. Each node along the path uses this information to associate the content with a specific area and the correspondent geoFace and to register the name-prefix~$\rightarrow$~GeoFace(s) pair in the FIB. %thus enabling the geographical interest forwarding even if the node is not actually running the specific application. 
%
% \begin{figure}
%%\vspace{-0.18in}
%\begin{minipage}[t!h]{\columnwidth}
%\centering
%\includegraphics[width=0.75\columnwidth]{GeoFace.png}
%%\vspace{-0.4cm}
%\caption{GeoFaces}
%\label{fig:GeoFace}
%\end{minipage}
%\vspace{-0.2in}
%\end{figure}

\subsection{System Model}
This paper is focused on urban scenarios. We assume all Vehicles equipped with a GPS sensor and a digital map, therefore able to identify their own location. Each vehicle is also equipped with wireless Ad-Hoc communication based on WiFi and with enough storage and computational capabilities; we leave the study of the performance under constrained caching to a future work.
Furthermore, we assume the presence of RSUs along some roads which provide Internet connectivity to all the cars and which are running a NDN stack and \nameNoSpace.
%%
%% LZ: this subsection is needed, but seems in a wrong place

%The urban scenario selected represents an area of Santa Monica, California, USA, the mobility traces are generated with SUMO\cite{SUMO2012} under the assumptions that major roads carry more traffic than residential ones. We are looking at relatively short commutes (i.e. 15 minutes or less) to match relatively small size of the area 2x2 km.  Roadside units (RSU) are positioned in the simulation theater to mimic the location of the actual access points deployed by Time Warner Cable in the same area; we selected only a subset of 4 out of the 21 access points currently deployed in that area~\cite{TWCwebsite}. The detailed simulation parameters are described in section \ref{sec:simulations}. In our model RSU are assumed to be  NDN nodes; no mac-layer  authentication or connection process are needed, we are aware that is far from the current  WiFi practices however newer standards such as  the vehicular specific IEEE802.11p~\cite{IEEE802.11p}  and the proposed IEEE802.11ai~\cite{IEEE802.11ai} do not require a MAC layer connection process to gain WiFi Access.  


%\subsection{Previous work: V-NDN}
%\todo{this section should briefly introduce V-NDN: LAL and V2VFace concepts. Maybe also few lines to say what we are adding }
%NDN has been deployed by ~\cite{2014NOM-VNDN}, which introduced  ... V2V face and LAL 




==> conclude.tex <==
% !TEX root = WoWMom.tex
\section{Conclusions}
\label{sec:conclude}


We developed a self-learning scheme to enable effective data delivery in highly dynamic vehicular environments.
\name takes advantage of the content geolocation to bind the name to the content area and to find the best path to guide the interest toward the data producers.  

\name has been evaluated through simulations and features low overhead and high performances for both V2V and V2I scenarios.
Our simulation setting assumes that all RSUs can listen to the packets within their vicinity of WiFi signal reachability.
We understand that the situation can be different in real WiFi deployment today, where RSUs may not be in the same SSID domain as vehicles and thus may not be able to receive/send packets with cars.
However this issue is simply the artifact of today's deployment, while our goal in this paper is to explore what is achievable by NDN based V2V, without the constraints of today's deployed base.

In contrast with IP-based geo-routing, which routes to a specific IP address, \name primarily routes towards content in a relatively large area. Furthermore, while IP-based geo-routing is connectivity-dependent and uses a one-hop hello protocol to maintain the local topology, while \name traffic in contrast is only related to the Interest--Data transactions, \ie{} if there are no consumers requesting content, there are no packets in the network.


==> introArx.tex <==
\section{Introduction}
\label{sec:intro}

Connectivity in a vehicular network is highly ad hoc. VANETs are made of dynamic, short lived links between vehicles that frequently come and go~\cite{rowstron2009characteristics}.  Traditional IP based node-to-node communication is a poor fit for the vehicular scenario because of the difficulties in coping with continuous disruptions and changes in network topology. 

Named Data Networking (NDN), in contrast, represents a radically different design.  An NDN network uses data names from applications directly for data delivery.  Because applications and their name spaces exist \emph{a priori}~\cite{VanSmThPlBriBra09-Networking}, NDN enables vehicles within vicinity of each other to exchange packets as soon as their signals can reach each other. Using application names eliminates the need for IP addresses.
However, in order to fetch data beyond the immediate neighborhood, vehicles need to make a decision on whether, and where, to forward Interests for specific content. 
In a wired network, this forwarding decision is assisted by NDN routing protocols which propagate data name prefixes throughout the network. In a vehicle network, data sources keep moving and connectivity changes frequently, making a routing protocol infeasible.

In this paper we describe \nameNoSpace, which exploits geographical information in place of a routing protocol to guide Interest forwarding in vehicular networks.  We develop solutions to (1) finding data sources' geographical information,
% which corresponds to a mapping between the content location and the name; 
and (2) forwarding Interests along the best paths, taking into account specific properties of the vehicle networking environment.
We evaluate our design through simulations.

Our contributions can be summarized as follows.
First, we developed effective solutions to the problem of mapping data names to data locations and forwarding Interest packets along the best path.
%% LZ: how is "best" defined here? 
Second, we designed an adaptive discovery and selection mechanism that can identify the available data sources across multiple geographic areas and can quickly react to sudden changes in vehicle networks. 
Third, our solution demonstrates the power of NDN architecture applied to vehicular networking and its ability to cope with ad hoc mobility and frequent network connectivity disruptions.
%Finally, we also identified remaining challenges. 

In the rest of the paper we first discuss the challenges in vehicular networking and identify the limitations in existing solutions in Section~\ref{sec:VANET-challenges.tex}.  We then sketch an overview of our solution in Section~\ref{sec:design}, and elaborate the design details in Sections~\ref{sec:forward} and~\ref{sec:LAL}).   Then we present the simulation scenarios and results in Section~\ref{sec:simulations}.  Lastly, we discuss and conclude the paper with some final remarks in Section~\ref{sec:discuss}.
%and conclude the paper with some final remarks in Section~\ref{sec:conclude}.



==> related.tex <==
\section{Related Work}
\label{sec:related}
\todo{maybe remove this entire section?}

earlier work (NOM 2012) assumed geo info embedded in data names. This is the case for certain classes of applications but not for all.

What other related work?



